MemDuet: Learning Dual-Process Memory for Long-Context Reasoning

Reasoning over infinitely long documents is becoming a reality with recurrent memory agents. However, increasing context length exacerbates the trade-off between reasoning performance and inference efficiency. Inspired by Kahneman's account of fast and slow thinking, we propose MemDuet, a dual-process memory framework that learns to coordinate a small language model for fast, parallel evidence selection from raw context chunks (System 1) with a large language model for memory-update verification and memory updates in document order (System 2). We train MemDuet in three stages: supervised fine-tuning of System 1 for evidence selection, Group Relative Policy Optimization (GRPO) of System 2 for verification and memory rewriting, and joint optimization of both policies to coordinate selection and updating for long-context reasoning. Experiments on diverse long-context reasoning benchmarks (RULER-HQA, LongBench v2, and 2WikiMultiHopQA) demonstrate a favorable accuracy-efficiency trade-off as context length grows. Averaged across evaluation settings on the three datasets, MemDuet achieves an end-to-end inference speedup of 9.74x and an output-token reduction of 73.91% relative to RL-MemAgent.

==> sections/s1_backbone_per_length_rows.tex <==
\midrule
\rowcolor{soneband}\multicolumn{12}{c}{\textit{Acc. (\%) $\uparrow$}}\\
\midrule
Qwen2.5-0.5B & 86.72 & 77.34 & 88.28 & 78.13 & 79.69 & 83.59 & 77.34 & 77.34 & 75.78 & 76.56 & 80.08 \\
Qwen2.5-1.5B & 86.72 & 84.38 & 89.06 & 82.03 & 85.16 & 82.81 & 82.03 & 79.69 & 78.91 & 78.13 & 82.89 \\
Qwen3.5-0.8B & 87.50 & 82.03 & 89.06 & 82.03 & 80.47 & 81.25 & 77.34 & 83.59 & 78.91 & 78.13 & 82.03 \\
\rowcolor{soneshade}Qwen3.5-2B & 87.50 & 83.59 & 89.06 & 79.69 & 87.50 & 85.94 & 82.81 & 82.03 & 79.69 & 75.78 & 83.36 \\
\midrule
\rowcolor{soneband}\multicolumn{12}{c}{\textit{Speed $\uparrow$}}\\
\midrule
Qwen2.5-0.5B & $0.826\times$ & $1.301\times$ & $1.458\times$ & $2.325\times$ & $2.911\times$ & $3.620\times$ & $5.926\times$ & $8.243\times$ & $11.186\times$ & $19.139\times$ & $5.69\times$ \\
Qwen2.5-1.5B & $0.791\times$ & $1.126\times$ & $1.477\times$ & $2.822\times$ & $3.749\times$ & $5.370\times$ & $7.977\times$ & $11.167\times$ & $17.636\times$ & $20.644\times$ & $7.28\times$ \\
Qwen3.5-0.8B & $0.791\times$ & $1.196\times$ & $1.642\times$ & $3.697\times$ & $6.812\times$ & $10.182\times$ & $15.961\times$ & $22.570\times$ & $34.407\times$ & $43.321\times$ & $14.06\times$ \\
\rowcolor{soneshade}Qwen3.5-2B & $0.983\times$ & $1.445\times$ & $1.588\times$ & $3.541\times$ & $5.885\times$ & $9.885\times$ & $11.913\times$ & $18.688\times$ & $39.085\times$ & $49.613\times$ & $14.26\times$ \\
\midrule
\rowcolor{soneband}\multicolumn{12}{c}{\textit{Tokens $\downarrow$}}\\
\midrule
Qwen2.5-0.5B & $.8645\times$ & $.5181\times$ & $.4256\times$ & $.2554\times$ & $.2028\times$ & $.1647\times$ & $.1001\times$ & $.0730\times$ & $.0557\times$ & $.0304\times$ & $.2690\times$ \\
Qwen2.5-1.5B & $.9012\times$ & $.5840\times$ & $.4045\times$ & $.1961\times$ & $.1452\times$ & $.1008\times$ & $.0678\times$ & $.0480\times$ & $.0287\times$ & $.0240\times$ & $.2500\times$ \\
Qwen3.5-0.8B & $.8963\times$ & $.5514\times$ & $.3658\times$ & $.1500\times$ & $.0736\times$ & $.0480\times$ & $.0283\times$ & $.0186\times$ & $.0100\times$ & $.0072\times$ & $.2149\times$ \\
\rowcolor{soneshade}Qwen3.5-2B & $.9050\times$ & $.5659\times$ & $.3671\times$ & $.2012\times$ & $.1154\times$ & $.0607\times$ & $.0543\times$ & $.0460\times$ & $.0117\times$ & $.0086\times$ & $.2336\times$ \\


==> sections/s1_backbone_summary_rows.tex <==
\configurationrow{white}{Qwen2.5-0.5B}{78.49}{80.08}{$5.69\times$}{$.2690\times$}
\configurationrow{white}{Qwen2.5-1.5B}{81.68}{82.89}{$7.28\times$}{$.2500\times$}
\configurationrow{white}{Qwen3.5-0.8B}{86.05}{82.03}{$14.06\times$}{$.2149\times$}
\configurationrow{memshade}{\blue{Qwen3.5-2B}}{84.47}{83.36}{$14.26\times$}{$.2336\times$}

